The World as a Graph: Improving El Ni\~no Forecasts with Graph Neural Networks

Deep learning-based models have recently outperformed state-of-the-art seasonal forecasting models, such as for predicting El Ni\~no-Southern Oscillation (ENSO). However, current deep learning models are based on convolutional neural networks which are difficult to interpret and can fail to model large-scale atmospheric patterns. In comparison, graph neural networks (GNNs) are capable of modeling large-scale spatial dependencies and are more interpretable due to the explicit modeling of information flow through edge connections. We propose the first application of graph neural networks to seasonal forecasting. We design a novel graph connectivity learning module that enables our GNN model to learn large-scale spatial interactions jointly with the actual ENSO forecasting task. Our model, \graphino, outperforms state-of-the-art deep learning-based models for forecasts up to six months ahead. Additionally, we show that our model is more interpretable as it learns sensible connectivity structures that correlate with the ENSO anomaly pattern.

==> figure_latex/diagram.tex <==
\begin{figure*}
 \centering
 \begin{subfigure}{0.8\textwidth}
  \centering
      \includegraphics[width=.9\textwidth]{figures/GNNs for ENSO_SLIDES.jpg}
  \end{subfigure}
\caption[diagram]{A diagram of our approach\salva{Where to put this figure?}}
\label{fig:diagram} 
\end{figure*}

==> sections/3_data.tex <==
%!TEX root=main.tex
 
\section{Data}\label{sec:data}

ENSO depends on and affects different environmental factors. Amongst these are sea-level pressure, zonal and meridional components of the surface wind, sea surface temperature, surface air temperature \cite{enso_complexity_timmermann2018}.
% \blmargin{*}{insert ref, e.g., an atmospheric sciences book w ENSO}
The climate variable, time series datasets of interest for this research are: \begin{itemize}
    \item 
    NOAA ERSSTv5\footnote{\href{https://psl.noaa.gov/data/gridded/data.noaa.ersst.v5.html}{ERSSTv5 data URL}},  with (partly reconstructed) SST data recorded since 1854, that we have used for initial setup and experiment,
    \item
    Coupled Model Intercomparison Project phase5 (CMIP5) historical simulations recorded since 1861, that are particularly interesting for pre-training the model since only few observational data are available,
    \item
    Simple Ocean Data Assimilation (SODA)\footnote{\href{https://coastwatch.pfeg.noaa.gov/erddap/griddap/hawaii_d90f_20ee_c4cb.html}{SODA data URL}}, reanalysis data recorded from 1870-2010,\blmargin{*}{i'd mention which measurements are you extracting from SODA and GODAS dataset? only SST?}
    \item
    Global Ocean Data Assimilation System (GODAS)\footnote{\href{https://psl.noaa.gov/data/gridded/data.godas.html}{GODAS data URL}} reanalysis data, recorded since 1980 only.
\end{itemize} 
% \blmargin{*}{Lots of datasets here. Be very precise and terse. Mention only the datasets you're planning to use and give one sentence on why.}
The last three datasets are open-source in the processed form they were used by \cite{CNN_ENSO} for pre-training, training and testing, respectively. 
The suitability of these datasets to deep learning methods has been demonstrated by \cite{CNN_ENSO}. Preliminary analysis will focus on these datasets, but more datasets may be incorporated to include other relevant variables, such as sea-level pressure and surface wind.

==> sections/7_Limitations.tex <==
% \section{Limitations}
%\vspace{-1mm}

%%%%%%%%%%%%%%%%%%%%%%% MOVED TO DISCUSSION ++++++++++++++++++++++++++++
% Limitations to our work include the potential influence of the seasonal cycle on our model. Information that reflects the seasonal cycle could be present in the data used to train the GNN2 model. This could be increasing our model’s performance if it is learning information pertinent to the seasonal cycle, rather than information unique to the ENSO phenomenon; which was a major criticism of \cite{CNN_ENSO}.

% A limitation of our model is the underestimation of the extreme ENSO events, as can be seen in Figure \ref{fig:timeseries}.
% By definition, these events are rare, which makes it a hard task for a ML model to correctly predict them from the limited sample size. The aforementioned seasonal cycle could be an additional factor causing this underestimation. A promising research direction may therefore focus on skillfully forecasting these extreme ENSOs, e.g supported by a custom loss function.\blXX{I like this paragraph. Maybe add a reference on anomaly prediction in time-series data?}
% While our model predicts most ENSO events with high skill, it predicts lower ONI indices for these extreme events. Discussions with Suyash Bire, a postdoctoral associate with a PhD in Marine and Atmospheric Science, has informed us this underestimation could be influenced by the model learning the seasonal cycle, and that removing this factor from the data and further tuning model hyperparameters could improve our model’s ability to predict extreme ENSO events.



==> sections/not_included/Not_Included.tex <==
%!TEX root=main.tex
\section{Appendix}\blXX{todo: rewrite, contains redundant information and unreferenced text}
\begin{figure}[t]
 \centering
 \begin{subfigure}{1.\columnwidth}
  \centering
      \includegraphics [trim=0 0 0 0.1in, clip, width=1.\textwidth, angle = 0]{figures/100_florence_harvey}
      \vspace{.02in}
      %\caption{Before training}
  \end{subfigure}
\caption[Unconditioned model]{Generated post-flooding imagery of the first $100$ tiles of the hurricane Harvey (left) and hurricane Florence (right) test set. \blXX{todo: mention in appendix}} \label{fig:100_florence_harvey} 
\end{figure}
\subsection{Dataset}\label{sec:appendix_dataset}
\subsubsection{Pre- and post-flood imagery}
Post-flood images that display standing water are challenging to acquire due to cloud-cover, time of standing flood, satellite revisit rate, and cost of high-resolution imagery. The xBD is the best publicly available data-source for high-resolution imagery of pre- and post-flood images at the time of writing (see Appendix or~\cite{Gupta_2019}.  
\begin{itemize}
    \item Data Overview: $3284$ flood-related image pairs from seven flood events at 1024x1024px of ~0.5m/px resolution of which 30\% display a standing flood (~1370)
    \item Flood-related events: hurricanes (Harvey, Florence, Michael, Matthew), spring floods (Midwest US, ‘19), tsunami (Indonesia), monsoon (Nepal)
    \item Our evaluation test set is composed by 108 images of hurricane Harvey, 108 of hurricane Florence. The test set excludes imagery from hurricane Michael or Matthew, because the majority of tiles does not display standing flood. % 98 of Hurricane Michael, and 73 of hurricane Matthew.
\end{itemize}
\subsubsection{Flood segmentations}
\blXX{Describe how flood segmentations have been created.}
For $\sim 100$ post-flood images, manually annotated segmentation masks of flooded/non-flooded pixels have been created. The labelled imagery will be made available at the project gitlab.

\subsubsection{Storm Surge predictions}
Developed by the National Weather Service (NWS), the Sea, Lake and Overland Surges from Hurricanes (SLOSH) model~\cite{Jelesnianski_92} estimates storm surge heights from atmospheric pressure, size, forward speed and track data, which are used as a wind model driving the storm surge. The SLOSH model consists of shallow water equations, which consider unique geographic locations, features and geometries. The model is run in deterministic, probabilistic and composite modes by various agencies for different purposes, including NOAA, National Hurricane Center (NHC) and NWS. We use outputs from the composite approach -- that is, running the model several thousand times with hypothetical hurricanes under different storm conditions. As a result, we obtain flood hazard map as displayed in (\cref{fig:related_works}, bot-left), “Storm Surge Prediction”, which are storm-surge, height-differentiated, flood extents. After implementing the SLOSH model into our workflow, we will use the state-of-the-art ADvanced CIRCulation model (ADCIRC)~\cite{Luettich_1992} model, which has a stronger physical foundation, better accuracy, and higher resolution than SLOSH. ADCIRC storm surge model output data is available for the USA from the Flood Factor online tool developed by First Street Foundation.

\subsection{Experiments}\label{sec:appendix_experiments}
Standard data augmentation, here rotation, random cropping, hue, and contrast variation \blXX{ask chris}, and state-of-the art augmentations target to satellite imagery, here elastic transformations (citation). Further spectral normalization has been used to ... And a relativistic loss function has been implemented to ... \blXX{TODO-table} shows the quantitative evaluation of these experiments, but shows the none of the experiments have increased performance. 
We trained Pix2pixhHD on LPIPS loss and not on physics-consistency loss (e.g., dice-sorensen, iou).

\textbf{Pre-training LPIPS on satellite imagery.} The standard LPIPS did not clearly distinguish in between the flood baseline and generated flood model, contrasting the opinion of a human evaluator. This is most likely because LPIPS currently leverages a neural network that was trained on object classification from ImageNet. The neural network might not be capable to extract meaningful high-level features to compare the similarity of satellite images. This was confirmed by preliminary tests in which the network would classify all satellite imagery as background image. Future work, will use LPIPS with a network trained to have satellite imagery specific features, e.g., Tile2Vec or a land-use segmentation~\cite{Robinson_2019} model. %Advanced: Modified FID with a feature space that is pretrained on a satellite imagery segmentation task, 
\blXX{add .. extending on~\cite{Zhou_2020}}

\blXX{todo:add thoughts on why high-res is necessary; add thought on climate change isn't v. visible}

